Compactifications of moduli of del Pezzo surfaces via line arrangement and K-stability

In this paper, we study compactifications of the moduli of smooth del Pezzo surfaces using K-stability and the line arrangement. We construct K-moduli of log del Pezzo pairs with sum of lines as boundary divisors, and prove that for $d=2,3,4$, these K-moduli of pairs are isomorphic to the K-moduli spaces of del Pezzo surfaces. For $d=1$, we prove that they are different by exhibiting some walls.

==> citation.tex <==


@article{CA21,
  title={The {C}alabi problem for {F}ano threefolds},
  author={Araujo, Carolina and Castravet, Ana-Maria and Cheltsov, Ivan and Fujita, Kento and Kaloghiros, Anne-Sophie and Martinez-Garcia, Jesus and Shramov, Constantin and Viswanathan, Nivedita and others},
  year={2021}
}


@article{BLX19,
  title={Openness of {K}-semistability for {F}ano varieties},
  author={Blum, Harold and Liu, Yuchen and Xu, Chenyang},
  journal={Duke Mathematical Journal},
  volume={171},
  number={13},
  pages={2753--2797},
  year={2022},
  publisher={Duke University Press}
}


@inproceedings{KRSS,
  title={Real space sextics and their tritangents},
  author={Kulkarni, Avinash and Ren, Yue and Sayyary Namin, Mahsa and Sturmfels, Bernd},
  booktitle={Proceedings of the 2018 ACM International Symposium on Symbolic and Algebraic Computation},
  pages={247--254},
  year={2018}
}

@article{LZ22,
  title={Equivariant K-stability under finite group action},
  author={Liu, Yuchen and Zhu, Ziwen},
  journal={International Journal of Mathematics},
  volume={33},
  number={01},
  pages={2250007},
  year={2022},
  publisher={World Scientific}
}

@article{HKT14,
  title={On the moduli of degree 4 Del Pezzo surfaces},
  author={Hassett, Brendan and Kresch, Andrew and Tschinkel, Yuri},
  journal={Development of moduli theory (Kyoto, 2013)},
  volume={69},
  pages={349--386},
  year={2013}
}


@article{Jia20,
  title={Boundedness of $\mb{Q}$-{F}ano varieties with degrees and alpha-invariants bounded from below},
  author={Chen Jiang},
  journal={Ann. Sci. Éc. Norm. Supér (4)},
  volume={53},
  number={5},
  pages={1235--1248},
  year={2020},
}


@article{LXZ22,
  title={Finite generation for valuations computing stability thresholds and applications to {K}-stability},
  author={Liu, Yuchen and Xu, Chenyang and Zhuang, Ziquan},
  journal={Annals of Mathematics},
  volume={196},
  number={2},
  pages={507--566},
  year={2022},
  publisher={Department of Mathematics of Princeton University}
}

@article{LWX21,
  title={Algebraicity of the metric tangent cones and equivariant {K}-stability},
  author={Li, Chi and Wang, Xiaowei and Xu, Chenyang},
  journal={Journal of the American Mathematical Society},
  volume={34},
  number={4},
  pages={1175--1214},
  year={2021}
}

@article{ABHLX20,
  title={Reductivity of the automorphism group of {K}-polystable {F}ano varieties},
  author={Alper, Jarod and Blum, Harold and Halpern-Leistner, Daniel and Xu, Chenyang},
  journal={Inventiones mathematicae},
  volume={222},
  number={3},
  pages={995--1032},
  year={2020},
  publisher={Springer}
}



@article{HKT09,
  title={Stable pair, tropical, and log canonical compactifications of moduli spaces of del Pezzo surfaces},
  author={Hacking, Paul and Keel, Sean and Tevelev, Jenia},
  journal={Inventiones mathematicae},
  volume={178},
  number={1},
  pages={173--227},
  year={2009},
  publisher={Springer}
}


@article{zha22,
  title={K-Moduli of Quintic Del Pezzo Pairs and Moduli of Genus Six Curves},
  author={Zhao, Junyan},
  journal={arXiv preprint arXiv:2212.06992},
  year={2022}
}


@article{Sko72,
  title={Sous-ensembles analytiques d’ordre fini ou infini dans $\mb{C}^n$},
  author={Skoda, Henri},
  journal={Bulletin de la Soci{\'{e}}t{\'{e}} Math{\'{e}}matique de France},
  volume={100},
  pages={353--408},
  year={1972}
}


@article{OSS16,
  title={Compact moduli spaces of del {P}ezzo surfaces and {K}{\"a}hler--{E}instein metrics},
  author={Odaka, Yuji and Spotti, Cristiano and Sun, Song},
  journal={Journal of Differential Geometry},
  volume={102},
  number={1},
  pages={127--172},
  year={2016},
  publisher={Lehigh University}
}


@book{KM98,
  title={Birational geometry of algebraic varieties},
  author={Koll{\'a}r, J{\'a}nos and Mori, Shigefumi},
  volume={134},
  year={1998},
  publisher={Cambridge university press}
}

@article{CS03,
  title={Recovering plane curves from their bitangents},
  author={Caporaso, Lucia and Sernesi, Edoardo},
  journal={J. Algebraic Geom.},
  volume={12},
  pages={225--244},
  year={2003}
}


@article{Tia87,
  title={On {K}{\"a}hler-{E}instein metrics on certain {K}{\"a}hler manifolds with $c_1(M)>0$},
  author={Tian, Gang},
  journal={Inventiones mathematicae},
  volume={89},
  number={2},
  pages={225--246},
  year={1987},
  publisher={Springer-Verlag}
}


@incollection{Fuj90,
  title={On singular del {P}ezzo varieties},
  author={Fujita, Takao},
  booktitle={Algebraic geometry},
  pages={117--128},
  year={1990},
  publisher={Springer}
}



@book{MFK94,
  title={Geometric invariant theory},
  author={Mumford, David and Fogarty, John and Kirwan, Frances},
  volume={34},
  year={1994},
  publisher={Springer Science \& Business Media}
}


@article{PT09,
  title={{CM} stability and the generalized {F}utaki invariant {II}},
  author={Paul, S. T. and Tian, G.},
  journal={Ast\'{e}risque},
  volume={328},
  pages={339--354},
  year={2009}
}

@article{GKS21,
  title={Geometric interpretation of toroidal compactifications of moduli of points in the line and cubic surfaces},
  author={Gallardo, Patricio and Kerr, Matt and Schaffler, Luca},
  journal={Advances in Mathematics},
  volume={381},
  pages={107632},
  year={2021},
  publisher={Elsevier}
}

@incollection{MM20,
  title={Stability and {E}instein-{K}{\"a}hler metric of a quartic del {P}ezzo surface},
  author={Mabuchi, Toshiki and Mukai, Shigeru},
  booktitle={Einstein metrics and Yang-Mills connections},
  pages={133--160},
  year={1993},
  publisher={CRC Press}
}



@article{AH81,
  title={Canonical curves and quadrics of rank 4},
  author={Arbarello, Enrico and Harris, Joseph},
  journal={Compositio mathematica},
  volume={43},
  number={2},
  pages={145--179},
  year={1981}
}


@article{LL19,
  title={K{\"a}hler--{E}instein metrics and volume minimization},
  author={Li, Chi and Liu, Yuchen},
  journal={Advances in Mathematics},
  volume={341},
  pages={440--492},
  year={2019},
  publisher={Elsevier}
}




@article{CP21,
  title={Positivity of the {CM} line bundle for families of {K}-stable klt {F}ano varieties},
  author={Codogni, Giulio and Patakfalvi, Zsolt},
  journal={Inventiones mathematicae},
  volume={223},
  number={3},
  pages={811--894},
  year={2021},
  publisher={Springer}
}


@article{LX19,
  title={K-stability of cubic threefolds},
  author={Liu, Yuchen and Xu, Chenyang},
  journal={Duke Mathematical Journal},
  volume={168},
  number={11},
  pages={2029--2073},
  year={2019},
  publisher={Duke University Press}
}



@book{Huy16,
  title={Lectures on {K}3 surfaces},
  author={Huybrechts, Daniel},
  volume={158},
  year={2016},
  publisher={Cambridge University Press}
}



@article{XZ20,
  title={On positivity of the {CM} line bundle on {K}-moduli spaces},
  author={Xu, Chenyang and Zhuang, Ziquan},
  journal={Annals of mathematics},
  volume={192},
  number={3},
  pages={1005--1068},
  year={2020},
  publisher={JSTOR}
}

@article{BLX22,
  title={Openness of {K}-semistability for {F}ano varieties},
  author={Blum, Harold and Liu, Yuchen and Xu, Chenyang},
  journal={Duke Mathematical Journal},
  volume={171},
  number={13},
  pages={2753--2797},
  year={2022},
  publisher={Duke University Press}
}


@article{Xu20,
  title={A minimizing valuation is quasi-monomial},
  author={Xu, Chenyang},
  journal={Annals of Mathematics},
  volume={191},
  number={3},
  pages={1003--1030},
  year={2020},
  publisher={Department of Mathematics of Princeton University}
}


@article{ADL19,
  title={Wall crossing for {K}-moduli spaces of plane curves},
  author={Ascher, Kenneth and DeVleming, Kristin and Liu, Yuchen},
  journal={arXiv preprint arXiv:1909.04576},
  year={2019}
}


@article{AK11,
  title={The moduli of curves of genus six and {K}3 surfaces},
  author={Artebani, Michela and Kond{\=o}, Shigeyuki},
  journal={Transactions of the American Mathematical Society},
  volume={363},
  number={3},
  pages={1445--1462},
  year={2011}
}



@article{Yan96,
  title={Sextic curves with simple singularities},
  author={Yang, Jin-Gen},
  journal={Tohoku Mathematical Journal, Second Series},
  volume={48},
  number={2},
  pages={203--227},
  year={1996},
  publisher={Mathematical Institute, Tohoku University}
}



@article{Has00,
  title={Local stable reduction of plane curve singularities},
  author={Hassett, Brendan},
  year={2000},
  journal={J. Reine Angew. Math.}, volume={520},
  pages={169--194}
}



@article{HW81,
  title={Normal {G}orenstein surfaces with ample anti-canonical divisor},
  author={Hidaka, Fumio and Watanabe, Kei-ichi},
  journal={Tokyo Journal of Mathematics},
  volume={4},
  number={2},
  pages={319--330},
  year={1981},
  publisher={Publication Committee for the Tokyo Journal of Mathematics}
}




@article{Gol21,
  title={Genus six curves, {K}3 surfaces, and stable pairs},
  author={Goluboff, J Ross},
  journal={International Mathematics Research Notices},
  volume={2021},
  number={13},
  pages={9908--9936},
  year={2021},
  publisher={Oxford University Press}
}



@article{ADL21,
  title={K-moduli of curves on a quadric surface and {K}3 surfaces},
  author={Ascher, Kenneth and DeVleming, Kristin and Liu, Yuchen},
  journal={Journal of the Institute of Mathematics of Jussieu},
  pages={1--41},
  year={2021},
  publisher={Cambridge University Press}
}


@article{FY17,
  title={Classification of log del {P}ezzo surfaces of index three},
  author={Fujita, Kento and Yasutake, Kazunori},
  journal={Journal of the Mathematical Society of Japan},
  volume={69},
  number={1},
  pages={163--225},
  year={2017},
  publisher={The Mathematical Society of Japan}
}


@article{Nak07,
  title={Classification of log del {P}ezzo surfaces of index two},
  author={Nakayama, Noboru},
  journal={J. Math. Sci. Univ. Tokyo},
  volume={14},
  number={3},
  pages={293--498},
  year={2007}
}




@article{Fuj19,
  title={A valuative criterion for uniform {K}-stability of $\mb{Q}$-{F}ano varieties},
  author={Fujita, Kento},
  journal={Journal f{\"u}r die reine und angewandte Mathematik (Crelles Journal)},
  volume={2019},
  number={751},
  pages={309--338},
  year={2019},
  publisher={De Gruyter}
}


@article{Li17,
  title={K-semistability is equivariant volume minimization},
  author={Li, Chi},
  journal={Duke Mathematical Journal},
  volume={166},
  number={16},
  pages={3147--3218},
  year={2017},
  publisher={Duke University Press}
}


@article{BX19,
  title={Uniqueness of {K}-polystable degenerations of {F}ano varieties},
  author={Blum, Harold and Xu, Chenyang},
  journal={Annals of Mathematics},
  volume={190},
  number={2},
  pages={609--656},
  year={2019},
  publisher={Department of Mathematics of Princeton University}
}



@article{Liu18,
  title={The volume of singular {K}{\"a}hler--{E}instein {F}ano varieties},
  author={Liu, Yuchen},
  journal={Compositio Mathematica},
  volume={154},
  number={6},
  pages={1131--1158},
  year={2018},
  publisher={London Mathematical Society}
}


@article{Fuj18,
  title={Optimal bounds for the volumes of {K}{\"a}hler-{E}instein {F}ano manifolds},
  author={Fujita, Kento},
  journal={American Journal of Mathematics},
  volume={140},
  number={2},
  pages={391--414},
  year={2018},
  publisher={Johns Hopkins University Press}
}



@article{Blu20,
  title={The normalized volume of a singularity is lower semicontinuous},
  author={Blum, Harold and Liu, Yuchen},
  journal={Journal of the European Mathematical Society},
  volume={23},
  number={4},
  pages={1225--1256},
  year={2020}
}


@article{LX18,
  title={Stability of valuations: higher rational rank},
  author={Li, Chi and Xu, Chenyang},
  journal={Peking Mathematical Journal},
  volume={1},
  number={1},
  pages={1--79},
  year={2018},
  publisher={Springer}
}

@article{Der16,
  title={On {K}-stability of finite covers},
  author={Dervan, Ruadha{\'\i}},
  journal={Bulletin of the London Mathematical Society},
  volume={48},
  number={4},
  pages={717--728},
  year={2016},
  publisher={Oxford University Press}
}

@article{KSB88,
  title={Threefolds and deformations of surface singularities},
  author={Koll{\'a}r, J{\'a}nos and Shepherd-Barron, Nicholas I},
  journal={Inventiones mathematicae},
  volume={91},
  number={2},
  pages={299--338},
  year={1988},
  publisher={Springer-Verlag}
}




@incollection{LLX20,
  title={A guided tour to normalized volume},
  author={Li, Chi and Liu, Yuchen and Xu, Chenyang},
  booktitle={Geometric analysis},
  pages={167--219},
  year={2020},
  publisher={Springer}
}


@article{Laz07,
  title={Deformations of singularities and variation of {GIT} quotients},
  author={Laza, Radu},
  journal={Transactions of the American Mathematical Society},
  volume={361},
  number={4},
  pages={2109--2161},
  year={2009}
}




@article{Has03,
  title={Moduli spaces of weighted pointed stable curves},
  author={Hassett, Brendan},
  journal={Advances in Mathematics},
  volume={173},
  number={2},
  pages={316--352},
  year={2003},
  publisher={Elsevier}
}


@article{Xu21,
  title={K-stability of {F}ano varieties: an algebro-geometric approach},
  author={Xu, Chenyang},
  journal={EMS Surv. Math. Sci.},
  volume={8},
  number={1},
  pages={265-354},
  year={2021},
}



@article{Zhu21,
  title={Optimal destabilizing centers and equivariant {K}-stability},
  author={Zhuang, Ziquan},
  journal={Inventiones mathematicae},
  volume={226},
  number={1},
  pages={195--223},
  year={2021},
  publisher={Springer}
}


 
